MULTISCRIPT: Multimodal Script Learning for Supporting Open Domain Everyday Tasks

Automatically generating scripts (i.e. sequences of key steps described in text) from video demonstrations and reasoning about the subsequent steps are crucial to the modern AI virtual assistants to guide humans to complete everyday tasks, especially unfamiliar ones. However, current methods for generative script learning rely heavily on well-structured preceding steps described in text and/or images or are limited to a certain domain, resulting in a disparity with real-world user scenarios. To address these limitations, we present a new benchmark challenge -- MultiScript, with two new tasks on task-oriented multimodal script learning: (1) multimodal script generation, and (2) subsequent step prediction. For both tasks, the input consists of a target task name and a video illustrating what has been done to complete the target task, and the expected output is (1) a sequence of structured step descriptions in text based on the demonstration video, and (2) a single text description for the subsequent step, respectively. Built from WikiHow, MultiScript covers multimodal scripts in videos and text descriptions for over 6,655 human everyday tasks across 19 diverse domains. To establish baseline performance on MultiScript, we propose two knowledge-guided multimodal generative frameworks that incorporate the task-related knowledge prompted from large language models such as Vicuna. Experimental results show that our proposed approaches significantly improve over the competitive baselines.

==> body/limitation.tex <==
\section{Limitations}
\subsection{Limitations of history step extractor}
We used a third-party library Katna to determine and extract keyframes for the history step extraction. Katna employs five visual-based algorithms for determining keyframes, without considering semantic factors. Given that the caption quality of the selected keyframes significantly impacts the overall quality of the prompts, we plan to investigate alternative, semantic-aware models for keyframe extraction in future work.
\subsection{Limitation of external knowledge prompter}
In the current task, the utilization of GPT2-XL\cite{radford2019language} as the external knowledge source may not be the most suitable choice. With the release of much larger pre-trained models, it has been noticed that the prompt quality of GPT2-XL does not meet the desired standards, leading to repetitive or irrelevant output. The incorporation of external knowledge can bring noise, particularly when the information is lacking in meaningful content or is not relevant to the target task. While a selector has been implemented to mitigate noise, the semantic-based estimation is not sufficient to effectively eliminate all types of noise.
\subsection{Limitation of hierarchically selective generator}
The intention to generate future steps of the current approach is insufficient, especially when the target step is less relevant to step history. In the current encoding approach, the step history and external knowledge for subsequent steps are not distinguished intentionally. We find that when the intent of previous steps is not strongly related to the subsequent ones, the model tends to repeat previous steps, even if the prompt offers a few subsequent step content.


==> body/problem.tex <==
\section{Problem Formulation}
%\lifu{whenever you write a sentence, be sure to go back to read it again and again to make sure it's fluent and there are no grammatical errors.}

%\lifu{Task-oriented multimodal next step generation?}



The \textit{task-oriented multimodal subsequent step generation task} aims to generate a subsequent step that is most likely to be taken to continue the target task, based on the goal of the task and the video demonstrating history actions. 
A $task$, such as \textit{baking bread}, \textit{putting on makeup}, and \textit{pruning plants}, is assumed to be achievable based on a sequence of stereotypical $steps$, where each $step$ describes a particular action and the objects involved, such as \textit{preheating the oven}, \textit{applying eyeliner}, \textit{cutting off the tops of plants}, and so on.

%is a sequence of $steps$ that are performed in a specific order to achieve a goal, such as baking bread, putting on makeup, pruning plants, etc. A $step$ is a specific action or operation required to complete a $task$, such as preheating the oven, applying eyeliner, and cutting off the tops of plants.

The input of \textbf{TASS} is a text-video pair $R$, which includes the task title $T$ in text format, and a video $V$ that introduces step history. It is important to note that video $V$ may include single or multiple previous steps in an individual and coherent video, so the number of completed steps and their corresponding video clips cannot be directly determined. The target output of TASS is a text sentence $S_{sub}$, describing the most likely step that will be performed next in order to continue finishing the task, formally as
\begin{equation}
    S_{sub} = argmax(P(S|R))
\end{equation}
